Supernova Legacy Survey: Using Spectral Signatures To Improve Type Ia Supernovae As Distance Indicators

GMOS optical long-slit spectroscopy at the Gemini-North telescope was used to classify targets from the Supernova Legacy Survey (SNLS) from July 2005 and May 2006 - May 2008. During this time, 95 objects were observed. Where possible the objects' redshifts (z) were measured from narrow emission or absorption features in the host galaxy spectrum, otherwise they were measured from the broader supernova features. We present spectra of 68 confirmed or probable SNe Ia from SNLS with redshifts in the range 0.17 \leq z \leq 1.02. In combination with earlier SNLS Gemini and VLT spectra, we used these new observations to measure pseudo-equivalent widths (EWs) of three spectral features - CaII H&K, SiII and MgII - in 144 objects and compared them to the EWs of low-redshift SNe Ia from a sample drawn from the literature. No signs of changes with z are seen for the CaII H&K and MgII features. Systematically lower EW SiII is seen at high redshift, but this can be explained by a change in demographics of the SNe Ia population within a two-component model combined with an observed correlation between EW SiII and photometric lightcurve stretch.

==> appa.tex <==
\section{Data Tables}

\begin{table*}
\begin{minipage}{150mm}
\caption{Table of observations. $^1$ Measured using GEMSEEING, $^2$ Measured using IMEXAM, $^3$ R150 observation, $^4$ Second night of data only used $^5$ First night of data only used}\label{obs_tab}
\begin{tabular}{c c c c c c c c}
\hline
SN & RA & Dec &UT Date& Exposure Time &Mode & $\lambda_{cent}$ & Seeing \footnotemark[1]\\
(SNLS name) & (J2000) & (J2000) & & (s) & &(nm) & ($''$)\\
\hline
05D4bo & 22:16:44.630 & -17:20:12.37 & 2005-07-14  & 2700 & N\&S & 720 & 0.43\\
06D1bt & 02:24:59:57 & -04:01:05.43 & 2006-08-31 & 5400 & N\&S & 720 & 0.45 \\
06D1bz & 02:25:07.62 & -04:42:06.58 & 2006-08-22 & 5400 & N\&S & 720 & 0.52 \\
06D1ck & 02:26:25.37 & -04:40:43.80 & 2006-08-31 & 3600 & N\&S & 720 & 0.40 \\
 &  &  &  2006-09-01 & 1800 & N\&S & 720 & 1.03\\
06D1dt & 02:27:15.20 & -04:35:44.88 & 2006-09-23 & 3600 & C & 680 & 0.51 \\
06D1gg & 02:26:28.56 & -04:44:54.29 & 2006-09-23 & 2400 & C  & 680 & 0.66\\
06D1gu & 02:24:33.91 & -04:17:37.80 & 2006-11-18 & 5400 & N\&S & 720 & 0.37\\
06D1hl & 02:26:42.95 & -04:18:22.34 & 2006-12-11 & 5400 & N\&S & 720 & 0.36\\
06D1jp & 02:25:48.07 & -04:17:56.02 & 2006-12-22 & 7200 & N\&S & 720 & 0.61\\
06D2iz & 10:00:34.76 & 02:19:20.17 & 2006-12-21 & 5400 & N\&S & 720 & 0.64\\
06D2ja & 10:00:33.51 & 02:28:01.01 & 2006-12-21 & 3600 & N\&S & 720 & 0.46 \\
06D2ji & 09:59:51.03 & 01:51:50.14 & 2006-12-19 & 7200 & N\&S & 720 & 0.66 \\
 &  &  &2006-12-20 & 1800 & N\&S & 720 & 0.38\\
06D2js & 10:02:15.70 & 02:35:06.62 & 2006-12-25 & 7200 & N\&S & 720 & 1.10\footnotemark[2] \\
06D2ju & 10:01:34.65 & 02:26:42.72 & 2006-12-24 & 5400 & N\&S & 720 & 0.83 \\
06D3ed & 14:18:47.82 & 52:45:23:28 & 2006-05-27 & 2400 & N\&S & 720 & 0.82 \\
06D3el & 14:17:01.06 & 52:13:56.84 & 2006-05-27 & 5400 & C & 680 & 0.72 \\
06D3et & 14:22:04.76 & 52:20:18.30 & 2006-05-31 & 5400 & N\&S & 720 & 0.56 \\
06D3fp & 14:20:18.62 & 52:53:49.62 & 2006-06-18 & 2600 & C & 680 & 0.55 \\
06D3fr & 14:19:20.24 & 52:31:50.11 & 2006-06-29 & 3600 & C & 680 & 1.07 \\
06D3fv & 14:21:03.31 & 53:00:52.77 & 2006-06-25 & 1800 & N\&S & 720 & 0.73 \\
 &  &  & 2006-06-29 & 5400 & N\&S & 720 & 0.65\\
06D3gg & 14:20:17.36 & 53:10:42.27 & 2007-07-20 & 3600 & N\&S & 720 &0.51 \\
06D3gh & 14:18:31.38 & 52:26:34.69 & 2006-06-30 & 5400 & N\&S & 720 & 0.41 \\
06D3gn & 14:17:44.61 & 52:21:40:42 & 2006-07-06 & 2700 & C & 680 & 0.40 \\
06D3gx & 14:17:03.36 & 52:56:21.82 & 2007-07-27 & 3600 & N\&S & 720 & 0.52 \\
06D3hd & 14:20:42.76 & 52:14:20.27 & 2006-07-18 & 3600 & C & 680 &0.72 \\
06D4dh & 22:14:19.70 & -17:35:06:23 & 2006-07-30 & 5400 & C & 680 & 0.51 \\
06D4dr & 22:16:46.00 & -17:20:45.49 & 2006-08-19 & 4800 & N\&S & 720 & 0.44 \\
06D4fc & 22:13:52.30 & -17:19:30.31 & 2006-09-23 & 5400 & N\&S & 720 & 0.39 \\
06D4fy & 22:14:06.22 & -17:34:19.34 & 2006-09-16 & 5400 & N\&S & 720 & 0.39 \\
06D4gn & 22:15:14.81 & -17:23:01.36 & 2006-09-22 & 7200 & N\&S & 720 & 0.42 \\
06D4hc & 22:15:40.52 & -18:09:08.71 & 2006-10-13 & 5400 & N\&S & 720 & 0.96 \\
07D1cx & 02:24:58.48 & -04:01:54.23 & 2007-11-10 & 3600 & N\&S & 720 & 0.44 \\
&&&&3600&  & 715\\
07D1ds & 02:25:24.44 & -04:18:49.29 & 2007-11-10 & 3600 & N\&S & 720 & 0.41 \\
&&&&3600&& 720\\
07D1dv & 02:26:51.27 & -04:47:18.29 & 2007-11-10 & 1800 & N\&S & 720 & 1.06 \\
&&&2007-11-11 & 1800 &&&0.51\\
&&&& 3600 &&715\\
07D1ea & 02:25:14:77 & -04:55:39.80 & 2007-11-13 & 3600 & N\&S & 720 & 0.45 \\
&&&& 3600 && 715\\
07D2bu & 09:59:27.590 & 02:33:03.48 & 2007-03-15 & 5400 &N\&S & 720 & 0.93 \\
&&& 2007-03-16 & 1800 & & & 0.63\\
&&& 2007-03-17 & 3600 & & & 0.77\\
07D2cy & 10:01:49.486  & 02:40:59.09  & 2007-03-22 & 3600 & N\&S & 720 & 0.82 \\
&&& 2007-03-22 & 5400 & & 715 & 0.51\\
07D2kc & 10:01:07.19 & 02:02:28.65 & 2007-12-20 & 900 & C & 680 & 0.67 \\
&&&& 1800&& 675\\
07D2ke & 10:01:04.73 & 01:59:31.81 & 2007-12-20 & 900 & C & 680 & 0.80 \\
&&&&900 && 675\\
07D2kh & 10:00:28.94 & 02:13:39.65 & 2008-01-04 & 3600 & N\&S & 720 & 0.63 \\
&&&& 1800 && 715\\
&&& 2008-01-06 & 1800 & && 0.32\\
07D2ki & 10:00:26.69 & 01:56:48.87 & 2008-01-05 & 3600 & N\&S & 720 & 0.54 \\
&&&& 1800 && 715\\
&&&2008-01-08 & 3600 &&&0.54\\
07D2kl & 09:59:16.95 & 02:31:28.13 & 2008-01-4 & 3600 & N\&S & 720 & 0.48 \\
&&&&3600 && 715\\
\end{tabular}
\end{minipage}
\end{table*}

\begin{table*}
\contcaption{}
\begin{minipage}{15cm}
\begin{tabular}{c c c c c c c c}
07D3ae & 14:17:33.70 & 52:31:27.17 & 2007-01-25 & 2400 & C & 680 & 0.57 \\
07D3af & 14:19:05.01 & 53:06:08.98 & 2007-01-27 & 2400 & C & 680 & 1.12\footnotemark[2] \\
07D3ai & 14:19:06.711 & 52:40:11.69 & 2007-02-14 & 3600 & C & 680 & 0.49 \\
07D3am & 14:22:36.55 & 52:20:26.26 & 2007-01-23 & 3600 & C & 680 & 0.70 \\
07D3ap & 14:18:10.26 & 52:23:07.38 & 2007-01-23 & 3600 & N\&S & 720 & 0.54 \\
07D3bb & 14:18:10.31 & 52:18:26.38 & 2007-01-25 & 7200 & N\&S & 720 & 0.46 \\
07D3bo & 14:20:58.408& 52:20:37.22  & 2007-02-14 & 5400 & N\&S & 720 & 0.54 \\
&&& 2007-02-15 & 1800 \\
07D3bp & 14:21:01.32 & 52:13:37.19 & 2007-01-27 & 7200 & B\&S & 720 & 0.75 \\
07D3bt & 14:21:25.719  & 52:58:13.67  & 2007-02-22 & 9000 & N\&S & 720 & 0.55 \\
07D3cn & 14:16:17.255 & 52:32:22.60  & 2007-03-24 & 3600 & N\&S & 720 & 0.50 \\
&&& 2007-03-25 & 5400 & & 715 & 0.41\\
07D3cr & 14:18:12.821 &52:19:04.57 & 2007-03-20 & 7200 & N\&S & 720 & 0.41 \\
07D3cu & 14:20:56.531 &52:15:13.36  & 2007-03-24 & 2400 & C & 680 & 0.49 \\
&&&& 2400 &&675 \\
07D3da & 14:20:06.236 & 52:16:16.64  & 2007-03-21 & 3600 & N\&S & 720 & 0.36 \\
&&&& 3600 & &715\\
07D3dj & 14:22:40.795 & 53:02:14.69  & 2007-04-12 & 3600 & C & 680 & 0.44 \\
07D3do & 14:20:35.683 & 52:44:48.58 & 2007-04-10 & 3600 & N\&S & 720 & 0.54\\
&&&& 3600 & &715\\
07D3ea & 14:21:16.116 &  52:40:07.88  & 2007-04-12 & 3600 & C & 680 & 0.47\\
&&& 2007-04-14 & 1200 & & &0.66\\
07D3ey\footnotemark[3] & 14: 19:18.944 & 53:04:35.92  & 2007-05-14 & 3600 & N\&S & 720 & 0.47 \\
&&&& 3600&&710\\
07D3fi\footnotemark[3] & 14:21:24.800 & 53:10:40.10  & 2007-04-23 & 3600 & N\&S & 720 & 0.77 \\
&&&& 3600 & &710\\
07D3gm\footnotemark[3] & 14:18:32.321 & 52:43:29.62 & 2007-05-19 & 3600 & N\&S & 720 & 0.47 \\
&&&& 3600&&710\\
07D3hl & 14:16:25.147 & 53:08:33.66& 2007-06-09 & 3600 & N\&S & 720 & 0.72 \\
&&&&3600&&715\\
07D3hu & 14:21:14.560 & 52:47:53.41 & 2007-06-11 & 3600 & N\&S & 720 & 0.37\\
&&&&1800&&715\\
07D3hv & 14:21:05.942 & 52:53:36.62 & 2007-06-11 & 3600 & C & 680 & 0.43 \\
07D3hw & 14:21:48.410 & 52:30:33.64 & 2007-06-08 & 3600 & N\&S & 720 & 0.53\\
&&&&3600&&715\\
07D3hz & 14:20:29.569 & 52:23:56.79 & 2007-06-10 & 3600 & C & 680 & 0.54 \\
07D3ib & 14:17:10.791 & 53:04:46.91 & 2007-06-16 & 3600 & N\&S & 720 & 0.74\\
&&&&1800&&715\\
&&&2007-06-18 & 1800 &&&0.89\\
07D3it & 14:18:08.730 & 52:25:04.06 & 2007-07-16 & 3600 & N\&S & 720 & 0.50 \\
&&&&3600&&715\\
07D4fl & 22:16:13.16 & -18:11:46.00 &2007-11-13 & 1800 & N\&S & 720 & 0.47 \\
&&&&3600 && 715\\
08D1aa \footnotemark[4]& 02:27:37.13 & -04:03:02.64 & 2008-01-27 & 1800 & N\&S & 720 & 0.69 \\
&&&&1800 && 715\\
&&&2008-02-13 & 1800 &&720 & 0.98\\
08D2aa \footnotemark[5]& 10:01:52.77 & 02:15:57.74 & 2008-01-15 & 1800 & N\&S & 720 &0.76\\
&&&2008-01-17 & 1800&&& 0.95\\
&&&&1800 && 715\\
08D2ad & 10:00:59.19 & 01:45:27.31 & 2008-01-09 & 1800 & N\&S & 720 & 0.60 \\
&&& 2008-01-10 & 3600\\
08D2au & 10:02:01.84 & 02:15:03.76 & 2008-01-17 & 1800 & N\&S & 720 & 0.60\\
&&&&1800 && 715\\
08D2bj \footnotemark[4]& 09:58:51.48 & 02:07:07.38 & 2008-01-10 & 3600 & N\&S & 720 & 0.42\\
&&&&3600 && 715 & 0.47\\
&&&2008-01-12 & 1800 &&715 \\
08D2ch & 10:01:39.61 & 02:06:57.56 & 2008-02-12 & 1800 & N\&S & 720 & 0.68 \\
&&&& 1800 && 715\\
08D2cl & 09:59:28.55 & 02:29:49.02 & 2008-02-12 & 3600 & N\&S & 720 & 0.94 \\
&&&& 1800 && 715\\
08D2dr & 10:01:54.13 & 02:04:01.96 & 2008-02-28 & 1200 & C & 680 & 0.66 \\
&&&& 1200 && 675\\
08D2dz & 09:58:53.07 & 01:44:19.21 & 2008-03-05 & 3600 & N\&S & 720 & 0.54 \\
&&&&3600 && 715\\
08D2eo & 10:02:03.85 & 02:33:44.74 & 2008-03-07 & 1200 & C & 680 & 0.51 \\
&&&&1200 && 675\\
\end{tabular}
\end{minipage}
\end{table*}


\begin{table*}
\contcaption{}
\begin{minipage}{15cm}
\begin{tabular}{c c c c c c c c}
08D2fj & 10:00:57:55 & 02:02:30.68 & 2008-03-09 & 1200 & C & 680 & 0.61 \\
&&&&1200 && 675\\
08D2gw & 10:01:05.95 & 02:31:19.93 & 2008-03-08 & 3600 & N\&S & 720 & 0.63\\
&&&& 1800 && 715\\
08D2hw & 10:00:06.70 & 02:33:08.66 & 2008-03-11 & 1800 & N\&S & 720 & 0.69 \\
&&&&3600 && 715\\
08D2id & 10:02:01.98 & 02:13:13.38 & 2008-04-02 & 1800 & N\&S & 720 & 0.60 \\
&&&&3600 && 715\\
08D2iq & 09:58:56.05 & 02:34:26.99 & 2008-04-08 & 1800 & N\&S & 720 & 0.45 \\
&&&&3600 && 715\\
08D2kj & 09:59:13.37 & 02:25:04.45 & 2008-04-08 & 3600 & N\&S & 720 & 0.43 \\
&&&& 3600 && 715\\
08D3au & 14:19:43.14 & 53:06:31.22 & 2008-02-15 & 1800 & N\&S & 720 & 0.61 \\
&&& 2008-02-17 & 3600 && 715 & 0.51\\
08D3bh & 14:17:06.50 & 53:01:37.38 & 2008-02-15 & 1800 & N\&S & 720 & 0.69 \\
&&&&1800 && 715\\
08D3dc & 14:20:44.79 & 52:46:48.15 & 2008-03-08 & 3600 & N\&S &720 & 0.51 \\
&&& 2008-03-10 & 3600 && 715 & 0.55\\
08D3dx & 14:17:47.82 & 52:23:02.76 & 2008-03-08 & 3600 & N\&S & 720 & 0.58 \\
&&&& 3600 && 715\\
08D3fp & 14:16:28.53 & 53:06:10.23 & 2008-04-08 & 3600 & N\&S & 720 & 0.64 \\
&&&& 3600 && 715\\
08D3fu & 14:22:35.86 & 53:00:36.98 & 2008-04-02 & 1800 & N\&S & 720 & 0.52 \\
&&&& 1800 && 715\\
08D3gb & 14:21:53.41 & 52:11:47.89 & 2008-04-03 & 1200 & C & 680 & 0.67 \\
&&&& 1200 && 675\\
08D3gf & 14:18:32.27 & 53:04:57.26 & 2008-04-12 & 1200 & C & 680 & 0.88 \\
&&&&1200 && 675\\
08D3gu & 14:21:24.10 & 53:05:35.12 & 2008-05-08 & 1800 & N\&S & 720 & 0.68 \\
&&&& 3600 && 715\\
08D3hh & 14:19:51.20 & 52:38:00.25 & 2008-05-12 & 1800 & N\&S & 720 & 0.49 \\
&&&& 3600 && 715\\
\hline
\end{tabular}
\end{minipage}
\end{table*}

\newpage

\begin{table*}
\begin{minipage}{12cm}
\caption{Classifications and redshifts.  Objects types are defined in Section \ref{sec:redshift-classification}}\label{res_tab}
\begin{tabular}{c c c c c c}
\hline
Target & Type & Redshift & Redshift Error & CI & Redshift Source \\
\hline
05D4bo & SN & ... & ... & 2 & ... \\
06D1bt & SNIa & 0.81 & 0.01 & 5 & target \\
06D1bz & SNIa & 0.833 & 0.001 & 4 & host \\
06D1ck & SNIa? & 0.90 & 0.02 & 3 & target \\
06D1dt & SN & 0.298 & 0.001 & 0 & target \\
06D1gg & SN & ... & ... & 1 & ... \\
06D1gu & SN & 0.87 & 0.01 & 2 & host \\
06D1hl & SN? & ... & ... & 2 & ... \\
06D1jp & SN & ... & ... & 2 & ... \\
06D2iz & SNIa? & 0.85 & 0.01 & 3 & target \\
06D2ja & SNIa & 0.726 & 0.001 & 4 & host \\
06D2ji & SNIa? & 0.90 & 0.01 & 3 & host \\
06D2js & SNIa & 0.60 & 0.01 & 5 & target \\
06D2ju & SNIa? & 0.927 & 0.001 & 3 & host \\
06D3ed & SNIa & 0.404 & 0.001 & 5 & host \\
06D3el & SNIa & 0.519 & 0.001 & 5 & host \\
06D3et & SNIa & 0.5755 & 0.0002 & 4 & host \\
06D3fp & SNIa & 0.268 & 0.001 & 5 & host \\
06D3fr & SNII & 0.275 & 0.001 & 0 & host \\
06D3fv & SN & ... & ... & 2 & ... \\
06D3gg & SNII & 0.2665 & 0.0003 & 0 & host \\
06D3gh & SNIa & 0.720 & 0.005 & 4 & host \\
06D3gn & SNIa & 0.2501 & 0.0002 & 5 & host \\
06D3gx & SNIa & 0.76 & 0.02 & 5 & target \\
06D3hd & SN & 0.2409 & 0.0002 & 2 & host \\
06D4dh & SNIa & 0.3027 & 0.0004 & 5 & host \\
06D4dr & SNIa & 0.76 & 0.01 & 5 & target \\
06D4fc & SNIa? & 0.677 & 0.001 & 3 & host \\
06D4fy & SNIa & 0.88 & 0.02 & 4 & target \\
06D4gn & SN & ... & ... & 2 & ... \\
06D4hc & SNII? & 0.38 & 0.01 & 1 & target \\
07D1cx & SNIa & 0.74 & 0.01 & 5 & target \\
07D1ds & SNIa & 0.706 & 0.001 & 4 & host \\
07D1dv & SNIa & 0.887 & 0.001 & 4 & host \\
07D1ea & SNIa & 0.775 & 0.001 & 5 & host \\
07D2bu & SN & 0.733 & 0.001 & 2 & host \\
07D2kc & SNIa & 0.354 & 0.001 & 4 & host \\
07D2ke & SNII & 0.114 & 0.001 & 0 & host \\
07D2kh & SNIa & 0.731 & 0.001 & 4 & host \\
07D2ki & SN? & 0.673 & 0.001 & 2 & host \\
07D2kl & SN? & 1.023 & 0.001 & 2 & host \\
07D2cy & SNIa & 0.886 & 0.001 & 4 & host \\
07D3ae & SNIa & 0.237 & 0.001 & 5 & host \\
07D3af & SNIa & 0.356 & 0.001 & 5 & host \\
07D3ai & SNII & 0.198 & 0.001 & 0 & host \\
07D3am & SNII & 0.214 & 0.001 & 0 & host \\
07D3ap & SNIa & 0.451 & 0.001 & 5 & host \\
07D3bb & SN? & ... & ... & 2 & ... \\
07D3bo & SNIa? & 0.92 & 0.02 & 3 & target \\
07D3bp & SN? & 0.769 & 0.001 & 2 & host \\
07D3bt & SNIa? & 0.91 & 0.01 & 3 & target \\
07D3cn & SNIa & 0.898 & 0.001 & 4 & host \\
07D3cr & SNIa & 0.746 & 0.001 & 4 & host \\
07D3cu & SNIa & 0.512 & 0.001 & 5 & host \\
07D3da & SNIa & 0.837 & 0.001 & 4 & host \\
07D3dj & SNIa & 0.444 & 0.001 & 5 & host \\
07D3do & SNIa? & 1.02 & 0.01 & 3 & target \\
07D3ea & SNIa & 0.471 & 0.001 & 5 & host \\
07D3ey & SNIa & 0.740 & 0.001 & 4 & host \\
07D3fi & SN & ... & ... & 2 & ... \\
07D3gm & SNIa & 0.83 & 0.02 & 5 & target \\
07D3hl & SNIa & 0.67 & 0.01 & 5 & target \\
\end{tabular}
\end{minipage}
\end{table*}

\begin{table*}
\contcaption{}
\begin{minipage}{12cm}
\begin{tabular}{c c c c c c}
07D3hu & SNIa & 0.572 & 0.001 & 4 & host \\
07D3hv & SNIa & 0.351 & 0.001 & 5 & host \\
07D3hw & SNIa & 0.748 & 0.001 & 5 & host \\
07D3hz & SNIa & 0.506 & 0.001 & 5 & host \\
07D3ib & SNIa & 0.681 & 0.001 & 4 & host \\
07D3it & SNIa & 0.835 & 0.001 & 4 & host \\
07D4fl & SNIa & 0.503 & 0.001 & 5 & host \\
08D1aa & SNIa? & 0.54 & 0.01 & 3 & target \\
08D2aa & SNIa & 0.538 & 0.001 & 5 & host \\
08D2ad & SNIa & 0.554 & 0.001 & 5 & host \\
08D2au & SN? & 0.563 & 0.001 & 2 & host \\
08D2bj & SNIa & 0.84 & 0.01 & 4 & target \\
08D2ch & SNIa? & 0.474 & 0.001 & 3 & host \\
08D2cl & SNIa? & 0.831 & 0.001 &3 & host \\
08D2dr & SNIa & 0.355 & 0.001 & 4 & host \\
08D2dz & SNIa & 0.65 & 0.01 & 4 & target \\
08D2eo & SNII & 0.125 & 0.001 & 0 & host \\
08D2fj & SN? & 0.507 & 0.001 & 1 & host \\
08D2gw & SNIa & 0.715 & 0.001 & 5 & host \\
08D2hw & SNIa & 0.746 & 0.001 & 4 & host \\
08D2id & SNIa & 0.833 & 0.001 & 4 & host \\
08D2iq & SNIa & 0.709 & 0.001 & 5 & host \\
08D2kj & SNIa & 0.702 & 0.001 & 5 & host \\
08D3au & SNII & ... & ... & 0 & ... \\
08D3bh & SNIa & 0.52 & 0.01 & 4 & target \\
08D3dc & SNIa & 0.799 & 0.001 & 5 & host \\
08D3dx & SNIa? & 0.928 & 0.001 & 3 & host \\
08D3fp & SN? & ... & ... & 2 & ... \\
08D3fu & SN? & 0.426 & 0.01 & 2 & target \\
08D3gb & SNIa & 0.17 & 0.01 & 5 & target \\
08D3gf & SNIa & 0.352 & 0.01 & 5 & host \\
08D3gu & SNIa & 0.767 & 0.001 & 5 & host \\
08D3hh & SNIa & 0.452 & 0.001 & 5 & host \\
\hline
\end{tabular}
\end{minipage}
\end{table*}

%% now we put in the EW data tables
\newpage
\begin{table*}
\begin{minipage}{8cm}
\caption{EW results for objects presented in this paper.  Objects marked * are removed from further analysis.}
\label{tab:walker_ew}
\begin{tabular}{c r@{$\pm$}l r@{$\pm$}l r@{$\pm$}l}
\hline
Object & \multicolumn{2}{c}{\protect\ion{Ca}{ii}} & \multicolumn{2}{c}{\protect\ion{Si}{ii}} & \multicolumn{2}{c}{\protect\ion{Mg}{ii}}\\
 & \multicolumn{2}{c}{(\AA)}&\multicolumn{2}{c}{(\AA)}&\multicolumn{2}{c}{(\AA)}\\
\hline
06D3ed & \multicolumn{2}{c}{--} & 6.13 & 6.16 & 95.37 & 15.52 \\
06D3el & 61.45 & 4.05 & 5.68 & 2.54 & 101.55 & 2.20 \\
06D3et & 89.26 & 5.87 & 17.57 & 3.09 & 55.34 & 4.05 \\
06D3fp & \multicolumn{2}{c}{--} & 18.78 & 3.21 & 108.85 & 0.89 \\
06D3gh & 103.48 & 8.15 & 3.78 & 4.02 & 155.73 & 10.23 \\
06D3gn & \multicolumn{2}{c}{--} & 27.65 & 4.91 & 102.63 & 6.63 \\
06D3gx & 94.55 & 14.06 & 11.82 & 4.37 & 87.19 & 17.48 \\
06D4dh & 27.98 & 5.04 & 5.79 & 0.53 & 68.54 & 0.68 \\
06D4dr & 106.78 & 8.31 & 23.25 & 3.03 & 99.13 & 6.25 \\
06D1bz & 122.01 & 9.01 & 10.56 & 5.56 & 114.96 & 12.12 \\
06D1bt & 89.71 & 6.89 & 2.78 & 4.82 & 13.76 & 8.99 \\
06D4fy* & 103.96 & 9.72 & 17.24 & 5.99 & -2.83 & 7.76 \\
06D2ja & 111.78 & 24.19 & 4.50 & 5.80 & 125.62 & 16.54 \\
06D2js & 92.66 & 15.41 & 24.67 & 3.38 & 148.98 & 7.53 \\
07D3ae & \multicolumn{2}{c}{--} & 25.97 & 5.22 & 128.72 & 4.77 \\
07D3da & 59.61 & 6.49 & 6.33 & 3.46 & 122.60 & 10.56 \\
07D2cy & 62.22 & 19.31 & 11.19 & 3.50 & 136.26 & 12.91 \\
07D3cn & 79.27 & 5.90 & 13.78 & 3.38 & 184.74 & 28.68 \\
07D3ea & 100.15 & 3.50 & 4.18 & 1.63 & 100.93 & 2.15 \\
07D3hw & 84.12 & 3.35 & 4.60 & 1.15 & 94.49 & 3.14 \\
07D3hl & 77.24 & 4.57 & 31.9 & 2.06 & 129.93 & 3.53 \\
07D3hv & 160.93 & 4.96 & 10.88 & 1.10 & 70.7 & 1.05 \\
07D3hu & 111.96 & 2.64 & 9.03 & 1.25 & 96.4 & 1.87 \\
07D3hz & 94.18 & 4.96 & 10.96 & 1.60 & 113.97 & 2.14 \\
07D3ib & 114.62 & 43.12 & 17.9 & 21.22 & 156.82 & 43.91 \\
07D3it & 49.31 & 14.42 & 28.04 & 9.76 & 147.35 & 16.35 \\
\hline
\end{tabular}
\end{minipage}
\end{table*}

\begin{table*}
\begin{minipage}{8cm}
\caption[EW results for the Bronder sample]{EW results for the Bronder sample.  Objects marked * are removed from further analysis}
\label{tab:bronder_ew}
\begin{tabular}{c r@{$\pm$}l r@{$\pm$}l r@{$\pm$}l}
\hline
Object & \multicolumn{2}{c}{\protect\ion{Ca}{ii}} & \multicolumn{2}{c}{\protect\ion{Si}{ii}} & \multicolumn{2}{c}{\protect\ion{Mg}{ii}}\\
 & \multicolumn{2}{c}{(\AA)}&\multicolumn{2}{c}{(\AA)}&\multicolumn{2}{c}{(\AA)} \\
\hline
03D1ax & 89.39 & 4.35 & 11.89 & 1.96 & 83.30 & 3.32 \\
03D1bk & 105.53 & 15.93 & 20.36 & 4.92 & 102.4 & 10.78 \\
03D1ew & 138.65 & 9.13 & 24.53 & 6.35 & 71.81 & 13.92 \\
03D1fq & 78.36 & 17.97 & 16.71 & 9.08 & 46.51 & 28.21 \\
03D4cn & 81.45 & 25.18 & 12.48 & 8.16 & 82.89 & 25.22 \\
03D4cy & 149.75 & 13.28 & 8.77 & 10.05 & 192.29 & 60.66 \\
03D4cz & 79.09 & 26.11 & 4.61 & 8.30 & 114.89 & 16.16 \\
03D4fd & 91.63 & 10.63 & 20.27 & 3.49 & 72.20 & 8.86 \\
03D4gl & 1.15 & 26.67 & 14.57 & 8.21 & 82.03 & 10.49 \\
04D1hd* & 138.83 & 47.54 & 9.4 & 10.61 & 1.62 & 14.68 \\
04D1hy & 140.26 & 21.38 & 15.57 & 5.10 & 104.05 & 12.32 \\
04D1ow & 137.96 & 8.54 & 23.02 & 6.43 & 91.12 & 13.65 \\
04D2ae & 159.04 & 21.44 & 5.0 & 13.16 & 102.02 & 24.69 \\
04D3dd & 124.99 & 34.38 & 44.63 & 28.33 & \multicolumn{2}{c}{--} \\
04D3fq & 93.32 & 27.30 & 29.09 & 16.44 & 113.69 & 30.91 \\
04D3kr & 115.8 & 3.07 & 17.65 & 2.43 & 104.62 & 4.12 \\
04D3lu & 69.35 & 8.48 & 8.47 & 4.92 & 127.63 & 14.53 \\
04D3ml & 98.52 & 3.5 & 12.75 & 3.68 & 136.11 & 6.12 \\
04D3nq & \multicolumn{2}{c}{--} & 9.32 & 26.37 & 113.18 & 22.69 \\
04D3ny & 108.34 & 16.28 & 21.19 & 13.69 & 80. & 29.84 \\
04D3oe & 30.14 & 8.61 & 11.10 & 3.11 & 74.93 & 7.59 \\
04D4dm & 121.67 & 37.87 & 7.91 & 14.98 & 108.92 & 39.95 \\
04D4gg & \multicolumn{2}{c}{--} & 3.49 & 6.33 & 99.97 & 15.97 \\
04D4hu & 61.65 & 16.73 & 9.73 & 5.65 & 91.93 & 11.00 \\
04D4ic & 69.98 & 56.30 & 15.22 & 22.33 & 125.52 & 48.55 \\
04D4ii & 121.3 & 13.19 & 1.22 & 10.87 & 117.13 & 30.69 \\
04D4im* & 108.27 & 14.24 & -0.23 & 2.99 & 157.3 & 8.69 \\
04D2mj & 104.52 & 10.11 & 9.88 & 4.30 & 54.16 & 6.55 \\
05D1az & 75.43 & 9.87 & 8.9 & 6.11 & 102.81 & 14.20 \\
05D1by & \multicolumn{2}{c}{--} & \multicolumn{2}{c}{--} & 89.15 & 9.26 \\
05D1cc & 48.66 & 11.90 & 17.57 & 5.77 & 81.48 & 14.97 \\
05D1ee & 54.87 & 11.85 & 0.09 & 4.69 & 104.43 & 12.22 \\
05D1em & 122.48 & 30.87 & 22.39 & 22.27 & 127.02 & 57.28 \\
05D2ab & \multicolumn{2}{c}{--} & 11.81 & 10.28 & 79.32 & 12.16 \\
05D2ah & \multicolumn{2}{c}{--} & \multicolumn{2}{c}{--} & 91.60 & 18.60 \\
05D2ck & 63.55 & 14.59 & 24.40 & 6.82 & 148.44 & 13.16 \\
05D2ja & \multicolumn{2}{c}{--} & 6.36 & 3.87 & 136.59 & 8.12 \\
05D2nt & 105.5 & 14.77 & 4.38 & 5.94 & 124.12 & 13.89 \\
05D2ob & 101.28 & 19.1 & 6.02 & 12.83 & 121.92 & 31.37 \\
05D3ax & 113.87 & 9.76 & 5.07 & 4.84 & 75.17 & 8.36 \\
05D3cf & \multicolumn{2}{c}{--} & 18.72 & 12.17 & 142.31 & 13.63 \\
05D3ci & 73.37 & 22.47 & 11.09 & 5.65 & 71.22 & 9.64 \\
05D3cx & 56.10 & 13.18 & 18.24 & 10.13 & 110.71 & 20.46 \\
05D3jq & 55.17 & 16.18 & 8.61 & 5.30 & 18.52 & 5.63 \\
05D3kt & 127.22 & 13.46 & 13.05 & 7.17 & 83.19 & 11.43 \\
05D3lb & 115.57 & 10.36 & 9.25 & 4.47 & 88.22 & 9.21 \\
05D3mh & 74.90 & 31.00 & 17.50 & 9.68 & 147.49 & 23.48 \\
05D3mq & \multicolumn{2}{c}{--} & 36.46 & 34.80 & 117.68 & 16.37 \\
05D3mx & 45.99 & 22.97 & 19.45 & 8.79 & 108.38 & 11.20 \\
05D4bm & 144.93 & 7.48 & 12.60 & 3.43 & 75.91 & 4.910 \\
05D4dt* & \multicolumn{2}{c}{--} & 2.13 & 2.64 & 6.38 & 3.17 \\
05D4dy & 95.96 & 25.01 & 23.12 & 11.81 & 125.51 & 23.31 \\
05D4fo & \multicolumn{2}{c}{--} & 28.59 & 4.52 & 80.82 & 5.90 \\
05D4gw & 143.8 & 27.02 & 12.85 & 10.66 & 131.23 & 21.20 \\
06D3bz & 113.9 & 21.40 & 13.48 & 9.22 & 81.48 & 24.17 \\
06D3cn & \multicolumn{2}{c}{--} & 6.57 & 2.6 & 103.29 & 0.93 \\
\hline
\end{tabular}
\end{minipage}
\end{table*}

\begin{table*}
\begin{minipage}{8cm}
\caption[EW results for the VLT sample]{EW results for the VLT sample.  Objects marked * are removed from further analysis.}
\label{tab:vlt_ew}
\begin{tabular}{c r@{$\pm$}l r@{$\pm$}l r@{$\pm$}l}
\hline
Object & \multicolumn{2}{c}{\protect\ion{Ca}{ii}} & \multicolumn{2}{c}{\protect\ion{Si}{ii}} & \multicolumn{2}{c}{\protect\ion{Mg}{ii}}\\
 & \multicolumn{2}{c}{(\AA)}&\multicolumn{2}{c}{(\AA)}&\multicolumn{2}{c}{(\AA)} \\
\hline
03D1bf & 81.38 & 30.45 & 14.90 & 15.42 & 133.44 & 34.85 \\
03D1co & 109.09 & 38.07 & 2.278 & 16.64 & 125.35 & 40.03 \\
03D1dt & 67.35 & 14.91 & 15.30 & 7.83 & 114.28 & 18.58 \\
03D1fc & 164.95 & 5.49 & 8.34 & 3.00 & 101.37 & 6.28 \\
03D1fl & 94.31 & 11.13 & 6.64 & 4.63 & 84.33 & 12.22 \\
03D4ag & 79.31 & 2.41 & 4.61 & 1.43 & 69.74 & 3.06 \\
03D4at & 97.01 & 18.06 & 5.67 & 9.12 & 90.27 & 28.34 \\
03D4au & 37.01 & 15.31 & 14.27& 9.00 & 31.70 & 17.43\\
03D4dy & 106.50 & 16.34 & 8.85 & 9.61 & 97.03 & 20.14 \\
04D1dc & 113.95 & 2.49 & 20.70 & 1.58 & 85.26 & 2.40 \\
04D1ff & 167.75 & 32.56 & 43.04 & 25.06 & \multicolumn{2}{c}{--} \\
04D1hx & 116.53 & 16.05 & 21.05 & 10.80 & 104.12 & 11.85 \\
04D1iv & 72.72 & 44.10 & \multicolumn{2}{c}{--} & \multicolumn{2}{c}{--} \\
04D1kj & 107.76 & 8.91 & 8.22 & 4.99 & 88.98 & 10.20 \\
04D1ks & 159.73 & 12.80 & 6.95 & 8.40 & 138.59 & 23.63 \\
04D1ow & 129.94 & 11.71 & 32.01 & 11.64 & \multicolumn{2}{c}{--} \\
04D1pd & 76.94 & 32.72 & 28.95 & 32.36 & \multicolumn{2}{c}{--} \\
04D1pg & 96.83 & 10.35 & 6.28 & 4.71 & 89.95 & 10.21 \\
04D1pp & 97.28 & 12.21 & 15.13 & 6.52 & 82.12 & 15.50 \\
04D1qd & 90.23 & 16.87 & 23.68 & 10.45 & \multicolumn{2}{c}{--} \\
04D1rh & 85.81 & 6.60 & 2.47 & 3.25 & 63.84 & 7.66 \\
04D1sa & \multicolumn{2}{c}{--} & 16.58 & 6.43 & 153.46 & 14.23 \\
04D1si & 84.13 & 16.46 & 22.00 & 10.35 & 147.02 & 23.31\\
04D2ac & 165.80 & 8.14 & 14.27 & 6.21 & 141.06 & 7.35 \\
04D2al & 123.58 & 32.75 & 26.08 & 24.54 & \multicolumn{2}{c}{--} \\
04D2an & 144.31 & 6.52 & 6.08 & 3.64 & 73.99 & 6.89 \\
04D2bt & 81.54 & 3.54 & 21.38 & 2.23 & 99.86 & 3.11 \\
04D2cf & 62.91& 5.47 & 3.09 & 3.71 & 94.26 & 16.80 \\
04D2fp & 126.43 & 4.39 & 9.90 & 4.26 & 70.24 & 12.53 \\
04D2fs & 132.86 & 2.88 & 14.32 & 1.85 & 94.73 & 3.98 \\
04D2gc & 58.41 & 8.54 & 1.69 & 3.66 & 92.56 & 10.47 \\
04D2gp & 104.44 & 16.43 & 24.44 & 7.34 & 134.22 & 15.70 \\
04D2mc* & \multicolumn{2}{c}{--} & -2.73 & 4.52 & 309.42 & 13.62 \\
04D4an & 62.89 & 13.99 & 20.31 & 8.01 & 61.90 & 18.72 \\
04D4bq & 110.81 & 8.08 & 23.95 & 5.74 & 124.34 & 7.62 \\
04D4fx & 116.50 & 7.85 & 0.10 & 3.30 & 109.84 & 9.82 \\
04D4ib & 65.19 & 17.47 & 3.98 & 6.26 & 114.75 & 12.89 \\
04D4jr & 97.73 & 3.62 & 3.92 & 2.35 & 85.73 & 5.19\\
04D4ju & 69.66 & 9.09 & 8.71 & 7.05 & 64.38 & 11.79 \\
05D1cb & 34.92 & 15.12 & 4.06 & 8.00 & 53.98 & 19.76 \\
05D1ck & 73.91 & 18.36 & 24.48 & 9.60 & 116.83 & 19.26 \\
05D1dn & 132.98 & 9.63 & 8.00 & 5.59 & 210.53 & 11.24 \\
05D2ac & 81.34 & 5.11 & 10.02 & 3.16 & 82.08 & 5.34 \\
05D2ay & 152.92 & 21.13 & 53.87 & 19.80 & \multicolumn{2}{c}{--} \\
05D2bt & 70.17 & 18.04 & 4.91 & 9.31 & 121.36 & 26.28 \\
05D2bv & 91.60 & 7.29 & 5.61 & 3.71 & 77.89 & 7.76 \\
05D2bw & 121.34 & 13.08 & 38.71 & 10.43 & \multicolumn{2}{c}{--} \\
05D2ci & 72.39 & 20.53 & 24.30 & 12.90 & 132.56 & 22.12 \\
05D2dt & 79.33 & 18.10 & 4.10 & 10.61 & 142.75 & 17.93 \\
05D2dw & 136.80 & 5.35 & 6.89 & 2.75 & 72.02 & 7.04 \\
05D2dy & 81.61 & 4.93 & 16.45 & 2.79 & 99.04 & 5.74 \\
05D2eb & 124.60 & 4.28 & 5.51 & 1.98 & 112.12 & 4.90 \\
05D2ec & 82.90 & 14.20 & 12.75 & 7.43 & 73.30 & 15.01 \\
05D2fq & 50.61 & 12.19 & 17.32 & 6.87 & \multicolumn{2}{c}{--} \\
05D2he & 117.27 & 15.70 & 12.54 & 8.51 & 114.48 & 15.64 \\
05D2ie & 74.94 & 6.19 & 7.05 & 3.34 & 60.53 & 9.98 \\
05D4af & 94.30 & 6.61 & 26.73 & 4.50 & 130.77 & 21.27 \\
05D4be & 69.84 & 5.65& 9.73 & 3.17 & 62.03 & 6.33 \\
05D4bi & 66.36 & 19.90 & 3.99 & 9.21 & \multicolumn{2}{c}{--} \\
05D4bj & 99.63 & 17.11 & 4.15 & 8.02 & 47.54 & 25.38 \\
05D4cq & 91.23 & 6.62 & 11.01 & 3.41 & 122.89 & 8.08 \\
05D4cs & 77.39 & 8.59 & 13.97 & 6.65 & 103.87 & 16.34 \\
05D4cw & 82.81 & 4.03& 6.02 & 2.57 & 103.19 & 6.08 \\
05D4dw & 81.49 & 29.46 & 35.37 & 32.32 & \multicolumn{2}{c}{--} \\
05D4ej & 52.77 & 11.41 & 3.03 & 6.44 & 83.65 & 11.16 \\
05D4ek & 121.09 & 13.43 & 16.47 & 5.41 & 92.95 & 10.24 \\
05D4ev & 160.49 & 15.43 & 29.04 & 7.47 & 83.67 & 16.07 \\
\hline
\end{tabular}
\end{minipage}
\end{table*}

% now low-z photometry and low-z EWs

\begin{table*}
\begin{minipage}{12cm}
\caption[Low-z Photometry]{Photometric properties of the low-z sample fitted using SiFTO}
\label{lowz_phot}
\begin{tabular}{c c r@{$ \pm $}l r@{$ \pm $}l r@{$ \pm $}l c}
\hline 
SN & Redshift\footnotemark[1] & \multicolumn{2}{c}{Stretch} & \multicolumn{2}{c}{Colour} & \multicolumn{2}{c}{B-band\footnotemark[2]}& Independent Distance \\ 
& &\multicolumn{2}{c}{} &\multicolumn{2}{c}{}& \multicolumn{2}{c}{(mag)}\\
\hline
SN\,1989B & 0.004 & 0.903 &  0.027 &  0.374 &  0.029 &  12.25 & 0.04 & 30.50 $\pm$ 0.09$^a$\\
SN\,1990N & 0.004 & 1.092 &  0.010 &  0.051 &  0.013 & 12.69 & 0.02 & 32.20 $\pm$ 0.09$^a$\\
SN\,1994D & 0.003 & 0.812 &  0.004 & -0.104 &  0.006 & 11.75 & 0.02 & 31.08 $\pm$ 0.20$^b$\\
SN\,1996X & 0.008 & 0.854 &  0.017 & -0.023 &  0.016 & 12.99 & 0.04 & -- \\
SN\,1998aq & 0.004 & 0.955 &  0.009 & -0.146 &  0.009  & 12.31 & 0.01 & 31.87 $\pm$ 0.15$^a$\\
SN\,1998bu & 0.004 & 0.954 &  0.016 &  0.262 &  0.011  & 12.11 & 0.02 & 30.34 $\pm$ 0.11$^a$\\
SN\,1999ee & 0.011 & 1.065 &  0.006 &  0.261 &  0.006  &  14.85 & 0.01 & -- \\
SN\,2000E & 0.004 & 1.060 &  0.012 &  0.128 &  0.035 & 12.85 & 0.15 & -- \\
SN\,2002bo & 0.005 & 0.942 &  0.011 &  0.379 &  0.014  & 13.95 & 0.02 & -- \\
SN\,2002er & 0.009 & 0.876 &  0.009 &  0.124 &  0.019  & 14.25 & 0.06 & -- \\
SN\,2003du & 0.007 & 1.006 &  0.007 & -0.112 &  0.008  & 13.46 & 0.01 & -- \\
SN\,2004eo & 0.015 & 0.869 &  0.005 &  0.048 &  0.013  & 15.07 & 0.05 & -- \\
SN\,2004S & 0.010 & 0.976 &  0.034 &  0.011 &  0.025 & 14.14 & 0.05 & -- \\
SN\,1997do & 0.010 & 0.944 &  0.029 &  0.002 &  0.027  & 14.27 & 0.05 & -- \\
SN\,1998V & 0.017 & 1.001 &  0.039 & -0.027 &  0.025 & 15.07 & 0.08 & -- \\
SN\,1998dh & 0.008 & 0.907 &  0.017 &  0.029 &  0.025  & 13.85 & 0.04 & -- \\
SN\,1998ec & 0.020 & 0.975 &  0.070 &  0.115 &  0.058  & 16.16 & 0.12 & -- \\
SN\,1998eg & 0.024 & 0.919 &  0.065 & -0.010 &  0.022  & 16.11 & 0.05 & -- \\
SN\,1999cc & 0.032 & 0.784 &  0.016 &  0.005 &  0.010  & 16.78 & 0.02 & -- \\
SN\,1999gd & 0.019 & 0.920 &  0.056 &  0.365 &  0.024  & 16.94 & 0.04 & -- \\
SN\,1999gp & 0.026 & 1.167 &  0.015 &  0.031 &  0.012  & 16.04 & 0.03 & -- \\
SN\,2000fa & 0.022 & 1.027 &  0.031 &  0.043 &  0.027  & 15.85 & 0.05 & -- \\
SN\,2001V & 0.016 & 1.128 &  0.012 &  0.050 &  0.015  & 14.62 & 0.02 & -- \\
\hline
\end{tabular}
\medskip
$^1$ Relative to CMB, $^2$ At date of maximum.\\
References: $^a$ \protect\citet{Saha:2006p2423} $^b$ \protect\citet{Ajhar:2001p2373}
\end{minipage}
\end{table*}

\begin{table*}
\begin{minipage}{8cm}
\caption{EW measurements for the low-z spectra.}\label{tab:lowz-ew}
\begin{tabular}{c c c c c}
\hline
Object & Phase &\ion{Ca}{ii} & \ion{Si}{ii} & \ion{Mg}{ii}\\
 & (Days) & (\AA) & (\AA) & (\AA)\\
\hline
SN\,1989B & 0 & -- & 26.56 & 98.58 \\
SN\,1989B & 6 & -- & 39.82 & 128.16 \\
SN\,1989B & 11 & -- & -- & 172.61 \\
SN\,1990N & -8 & -- & 6.92 & 92.35 \\
SN\,1990N & 2 & -- & 15.44 & 80.78 \\
SN\,1994D & -11 & 193.27 & 10.09 & 59.06 \\
SN\,1994D & -9 & -- & 15.13 & 68.78 \\
SN\,1994D & -8 & -- & 20.16 & 57.26 \\
SN\,1994D & -5 & 100.77 & 20.10 & 65.99 \\
SN\,1994D & -4 & 96.37 & 18.09 & 74.21 \\
SN\,1994D & -2 & 99.63 & 23.05 & 79.46 \\
SN\,1994D & 2 & 63.20 & 23.45 & 71.85 \\
SN\,1994D & 4 & 75.34 & 21.47 & 65.94 \\
SN\,1994D & 10 & -- & 20.39 & 90.39 \\
SN\,1994D & 11 & 65.92 & 16.71 & 108.98 \\
SN\,1996X & -2 & 41.29 & 17.18 & 86.65 \\
SN\,1996X & 0 & 81.01 & 17.77 & 92.88 \\
SN\,1996X & 1 & 82.05 & 17.75 & 91.66 \\
SN\,1996X & 7 & 80.56 & 13.71 & 93.10 \\
SN\,1998aq & -9 & 29.61 & 10.29 & 92.22 \\
SN\,1998aq & -8 & 58.20 & 10.27 & 95.58 \\
SN\,1998aq & 1 & 38.40 & 10.18 & 79.06 \\
SN\,1998aq & 2 & 38.79 & 12.37 & 81.56 \\
SN\,1998aq & 3 & 37.22 & 12.01 & 94.22 \\
SN\,1998aq & 4 & 38.15 & 12.78 & 96.98 \\
SN\,1998aq & 5 & 40.50 & 12.70 & 94.88 \\
SN\,1998aq & 6 & 40.15 & 12.61 & 96.50 \\
SN\,1998aq & 7 & 39.76 & 12.88 & 95.41 \\
SN\,1998bu & -4 & 91.48 & 15.24 & 99.23 \\
SN\,1998bu & -3 & 89.16 & 15.24 & 99.23 \\
SN\,1998bu & -2 & 87.53 & 14.30 & 98.41 \\
SN\,1998bu & 8 & 81.97 & 15.27 & 90.43 \\
SN\,1998bu & 9 & 83.49 & 16.36 & 91.26 \\
SN\,1998bu & 10 & 86.99 & 14.78 & 96.61 \\
SN\,1998bu & 11 & 82.38 & 13.68 & 112.96 \\
SN\,1999ee & -11 & 95.76 & 1.14 & 106.85 \\
SN\,1999ee & -9 & 98.16 & 1.75 & 93.78 \\
SN\,1999ee & -4 & 103.10 & 7.29 & 104.13 \\
SN\,1999ee & -2 & 108.93 & 7.92 & 102.26 \\
SN\,1999ee & 0 & 109.82 & 8.91 & 105.23 \\
SN\,1999ee & 5 & 129.76 & 18.67 & 112.07 \\
SN\,1999ee & 7 & -- & 20.11 & 114.87 \\
SN\,1999ee & 9 & 132.32 & 13.38 & 114.11 \\
SN\,2000E & -9 & 148.74 & 9.88 & 105.79 \\
SN\,2000E & -5 & -- & 9.97 & 82.18 \\
SN\,2000E & 5 & 142.57 & 12.86 & 91.46 \\
SN\,2002bo & -11 & 195.34 & 20.38 & 107.06 \\
SN\,2002bo & -6 & 152.29 & 17.78 & 105.13 \\
SN\,2002bo & -5 & 191.09 & 23.85 & 109.45 \\
SN\,2002bo & -4 & 137.57 & 22.08 & 104.52 \\
SN\,2002bo & -3 & 137.96 & 22.85 & 104.29 \\
SN\,2002bo & -2 & 142.47 & 33.86 & 114.94 \\
SN\,2002bo & -1 & 145.12 & 23.34 & 108.19 \\
SN\,2002bo & 4 & 118.94 & 36.97 & 117.07 \\
SN\,2002er & -11 & 170.87 & 23.61 & 107.01 \\
SN\,2002er & -9 & -- & 27.09 & 102.27 \\
SN\,2002er & -8 & 168.78 & 22.12 & 98.25 \\
SN\,2002er & -7 & 179.28 & 39.70 & 99.45 \\
SN\,2002er & -6 & 161.45 & 20.32 & 102.01 \\
SN\,2002er & -5 & 162.72 & 20.72 & 103.20 \\
SN\,2002er & -4 & 171.20 & 23.61 & 105.90 \\
SN\,2002er & -3 & 152.98 & 19.58 & 91.61 \\
SN\,2002er & -2 & 152.98 & 19.58 & 91.61 \\
\end{tabular}
\end{minipage}
\end{table*}

\begin{table*}
\contcaption{}
\begin{minipage}{8cm}
\begin{tabular}{c c c c c}
SN\,2002er & -1 & 149.57 & 22.05 & 97.47 \\
SN\,2002er & 0 & -- & 21.51 & 115.32 \\
SN\,2002er & 2 & -- & 23.78 & 97.44 \\
SN\,2002er & 4 & 111.98 & 25.90 & 99.99 \\
SN\,2002er & 5 & -- & 35.25 & 128.83 \\
SN\,2002er & 6 & 108.88 & 24.68 & 88.57 \\
SN\,2002er & 10 & 108.03 & 8.29 & 110.61 \\
SN\,2003du & -11 & 145.34 & 17.62 & 82.77 \\
SN\,2003du & -8 & 176.57 & 14.33 & 92.39 \\
SN\,2003du & -7 & 155.24 & 12.39 & 93.97 \\
SN\,2003du & -6 & 134.42 & 10.66 & 82.10 \\
SN\,2003du & -4 & 133.97 & 12.75 & 83.85 \\
SN\,2003du & -2 & 132.71 & 12.15 & 89.28 \\
SN\,2003du & -1 & 138.70 & 12.40 & 90.29 \\
SN\,2003du & 0 & 136.87 & 13.52 & 93.04 \\
SN\,2003du & 1 & 141.85 & 14.25 & 93.59 \\
SN\,2003du & 3 & 134.86 & 14.39 & 80.77 \\
SN\,2003du & 4 & 119.98 & 14.63 & 79.39 \\
SN\,2003du & 7 & 89.99 & 16.42 & 85.42 \\
SN\,2003du & 8 & 89.31 & 15.90 & 82.90 \\
SN\,2003du & 9 & 86.63 & 17.18 & 84.06 \\
SN\,2003du & 10 & 85.06 & 16.99 & 88.40 \\
SN\,2004dt & -10 & 81.19 & 43.41 & 118.9 \\
SN\,2004dt & -9 & 89.76 & 40.28 & 119.82 \\
SN\,2004dt & -7 & 91.64 & 34.27 & 109.54 \\
SN\,2004dt & -6 & 97.04 & 30.46 & 115.12 \\
SN\,2004dt & -4 & 97.79 & 27.33 & 113.16 \\
SN\,2004dt & -3 & 96.84 & 32.15 & 130.73 \\
SN\,2004dt & -2 & 98.46 & 24.45 & 120.35 \\
SN\,2004dt & -1 & 116.19 & 20.96 & 104.04 \\
SN\,2004dt & 2 & 120.69 & 25.87 & 99.30 \\
SN\,2004dt & 3 & 131.45 & 24.94 & 115.57 \\
SN\,2004eo & -6 & 136.35 & 24.30 & 107.61 \\
SN\,2004eo & -3 & 118.77 & 32.41 & 128.00 \\
SN\,2004eo & 2 & 96.18 & 25.44 & 104.67 \\
SN\,2004eo & 7 & 92.51 & 15.36 & 130.34 \\
SN\,2004S & 1 & 148.99 & 10.46 & 110.43 \\
SN\,2004S & 7 & 144.40 & 13.59 & 121.01 \\
SN\,1997do & -11 & -- & 14.33 & 105.19 \\
SN\,1997do & -10 & -- & 12.12 & 97.86 \\
SN\,1997do & -7 & -- & 20.44 & 113.20 \\
SN\,1997do & -6 & -- & 15.18 & 103.68 \\
SN\,1997do & 8.5 & -- & 11.52 & 101.07 \\
SN\,1997do & 10.5 & -- & 11.94 & 123.93 \\
SN\,1998V & 0.5 & -- & 14.54 & 92.82 \\
SN\,1998V & 1.5 & -- & 16.38 & 103.11 \\
SN\,1998V & 2.5 & -- & 13.64 & 90.24 \\
SN\,1998dh & -9 & -- & 24.87 & 102.04 \\
SN\,1998dh & -8 & -- & 26.35 & 105.01 \\
SN\,1998dh & -7 & -- & 24.21 & 105.78 \\
SN\,1998dh & -5 & -- & 27.31 & 110.46 \\
SN\,1998dh & -3 & -- & 30.62 & 107.46 \\
SN\,1998dh & 0 & -- & 27.46 & 109.28 \\
SN\,1998ec & -2.5 & -- & 23.23 & 115.56 \\
SN\,1998ec & -1.5 & -- & 18.02 & 109.87 \\
SN\,1998eg & 0 & -- & 22.23 & 98.36 \\
SN\,1998eg & 5 & -- & 24.91 & 106.30 \\
SN\,1999cc & -3 & -- & 32.39 & 107.29 \\
SN\,1999cc & -1 & -- & 32.82 & 112.07 \\
SN\,1999cc & 0.5 & -- & 26.97 & 116.27 \\
SN\,1999cc & 2 & -- & 34.46 & 108.90 \\
SN\,1999ej & -0.5 & -- & 28.54 & 91.06 \\
SN\,1999ej & 2.5 & -- & 27.16 & 91.83 \\
SN\,1999ej & 4.5 & -- & 22.25 & 90.77 \\
SN\,1999ej & 9 & -- & 16.85 & 123.35 \\
\end{tabular}
\end{minipage}
\end{table*}

\begin{table*}
\contcaption{}
\begin{minipage}{8cm}
\begin{tabular}{c c c c c}
SN\,1999gd & 2.5 & -- & 36.35 & 117.13 \\
SN\,1999gd & 9.5 & -- & 26.53 & 104.11 \\
SN\,1999gp & -4.5 & -- & 6.28 & 111.09 \\
SN\,1999gp & -1.5 & -- & 5.55 & 107.13 \\
SN\,1999gp & 0.5 & -- & 10.44 & 89.89 \\
SN\,1999gp & 3 & -- & 9.64 & 109.73 \\
SN\,1999gp & 5 & -- & 22.98 & 125.49 \\
SN\,1999gp & 7 & -- & 24.69 & 114.61 \\
SN\,2000fa & -10 & -- & 12.55 & 102.34 \\
SN\,2000fa & 1.5 & -- & 25.13 & 120.30 \\
SN\,2000fa & 2.5 & -- & 17.96 & 100.17 \\
SN\,2000fa & 4.5 & -- & 19.19 & 105.09 \\
SN\,2000fa & 9.5 & -- & 25.16 & 99.18 \\
SN\,2001V & -11 & -- & 10.01 & 82.89 \\
SN\,2001V & -10 & -- & 7.81 & 79.05 \\
SN\,2001V & -9.5 & -- & 7.98 & 81.46 \\
SN\,2001V & -7.5 & -- & 12.15 & 96.19 \\
SN\,2001V & -6.5 & -- & 12.07 & 98.80 \\
SN\,2001V & -5.5 & -- & 10.11 & 94.55 \\
SN\,2001V & -3.5 & -- & 9.10 & 89.31 \\
SN\,2001V & 9.5 & -- & 15.82 & 92.23 \\
SN\,2001V & 10.5 & -- & 19.66 & 93.89 \\
\hline
\end{tabular}
\end{minipage}
\end{table*}

\clearpage

%%% Local Variables:  %%% mode: latex %%% TeX-master: "snls_spec_v3" %%% End: 

==> appb.tex <==

\section{High-z Spectra}\label{sec:high-z-spectra}

Here we present all the SNLS supernova candidates observed at Gemini  between  May 2006 -- May 2008.  The spectra show the raw data in light blue with a smoothed version in dark blue.  The smoothing is done using a Savitzky-Golay smoothing filter \citep{citeulike:4226570}.  The spectra are grouped according to their classifications.  In the data plots, if any separate host galaxy extraction was possible it is  plotted in green.  Any narrow lines from host emission/absorption are marked.  The results of galaxy template subtraction from the method presented in Section \ref{sec:methods-measurements} are plotted in red.

\newpage


\begin{figure*}
\begin{center}
\subfigure[06D1bt $z=0.81$]{
\includegraphics[scale=0.40]{06D1bt_data2.eps}
\label{subfig:06D1bt_data2}
}
\subfigure[06D1bz $z=0.833$]{
\includegraphics[scale=0.40]{06D1bz_data2.eps}
\label{subfig:06D1bz_data2}
}
\subfigure[06D2ja $z=0.726$]{
\includegraphics[scale=0.40]{06D2ja_data2.eps}
\label{subfig:06D2ja_data2}
}
\subfigure[06D2js $z=0.60$]{
\includegraphics[scale=0.40]{06D2js_data2.eps}
\label{subfig:06D2js_data2}
}
\subfigure[06D3ed $z=0.404$]{
\includegraphics[scale=0.40]{06D3ed_data2.eps}
\label{subfig:06D3ed_data2}
}
\subfigure[06D3el $z=0.519$]{
\includegraphics[scale=0.40]{06D3el_data2.eps}
\label{subfig:06D3el_data2}
}
\subfigure[06D3et $z=0.5755$]{
\includegraphics[scale=0.40]{06D3et_data2.eps}
\label{subfig:06D3et_data2}
}
\subfigure[06D3fp $z=0.268$]{
\includegraphics[scale=0.40]{06D3fp_data2.eps}
\label{subfig:06D3fp_data2}
}
\end{center}
\caption{Type Ia Supernovae (CI = 4 or 5)}
\end{figure*}


\begin{figure*}
\begin{center}
\subfigure[06D3gh $z=0.720$]{
\includegraphics[scale=0.40]{06D3gh_data2.eps}
\label{subfig:06D3gh_data2}
}
\subfigure[06D3gn $z=0.2501$]{
\includegraphics[scale=0.40]{06D3gn_data2.eps}
\label{subfig:06D3gn_data2}
}
\subfigure[06D3gx $z=0.76$]{
\includegraphics[scale=0.40]{06D3gx_data2.eps}
\label{subfig:06D3gx_data2}
}
\subfigure[06D4dh $z=0.3027$]{
\includegraphics[scale=0.40]{06D4dh_data2.eps}
\label{subfig:06D4dh_data2}
}
\subfigure[06D4dr $z=0.76$]{
\includegraphics[scale=0.40]{06D4dr_data2.eps}
\label{subfig:06D4dr_data2}
}
\subfigure[06D4fy $z=0.88$]{
\includegraphics[scale=0.40]{06D4fy_data2.eps}
\label{subfig:06D4fy_data2}
}
\subfigure[07D1cx $z=0.74$]{
\includegraphics[scale=0.40]{07D1cx_data2.eps}
\label{subfig:07D1cx_data2}
}
\subfigure[07D1ds $z=0.706$]{
\includegraphics[scale=0.40]{07D1ds_data2.eps}
\label{subfig:07D1ds_data2}
}
\end{center}
\caption{Type Ia Supernovae (CI = 4 or 5)}
\end{figure*}


\begin{figure*}
\begin{center}
\subfigure[07D1dv $z=0.887$]{
\includegraphics[scale=0.40]{07D1dv_data2.eps}
\label{subfig:07D1dv_data2}
}
\subfigure[07D1ea $z=0.775$]{
\includegraphics[scale=0.40]{07D1ea_data2.eps}
\label{subfig:07D1ea_data2}
}
\subfigure[07D2kc $z=0.354$]{
\includegraphics[scale=0.40]{07D2kc_data2.eps}
\label{subfig:07D2kc_data2}
}
\subfigure[07D2kh $z=0.731$]{
\includegraphics[scale=0.40]{07D2kh_data2.eps}
\label{subfig:07D2kh_data2}
}
\subfigure[07D2cy $z=0.886$]{
\includegraphics[scale=0.40]{07D2cy_data2.eps}
\label{subfig:07D2cy_data2}
}
\subfigure[07D3ae $z=0.237$]{
\includegraphics[scale=0.40]{07D3ae_data2.eps}
\label{subfig:07D3ae_data2}
}
\subfigure[07D3af $z=0.237$]{
\includegraphics[scale=0.40]{07D3af_data2.eps}
\label{subfig:07D3af_data2}
}
\subfigure[07D3ap $z=0.451$]{
\includegraphics[scale=0.40]{07D3ap_data2.eps}
\label{subfig:07D3ap_data2}
}
\end{center}
\caption{Type Ia Supernovae (CI = 4 or 5)}
\end{figure*}


\begin{figure*}
\begin{center}
\subfigure[07D3cn $z0.898$]{
\includegraphics[scale=0.40]{07D3cn_data2.eps}
\label{subfig:07D3cn_data2}
}
\subfigure[07D3cr $z-0.746$]{
\includegraphics[scale=0.40]{07D3cr_data2.eps}
\label{subfig:07D3cr_data2}
}
\subfigure[07D3cu $z=0.512$]{
\includegraphics[scale=0.40]{07D3cu_data2.eps}
\label{subfig:07D3cu_data2}
}
\subfigure[07D3da $z=0.837$]{
\includegraphics[scale=0.40]{07D3da_data2.eps}
\label{subfig:07D3da_data2}
}
\subfigure[07D3dj $z=0.444$]{
\includegraphics[scale=0.40]{07D3dj_data2.eps}
\label{subfig:07D3dj_data2}
}
\subfigure[07D3ea $z=0.471$]{
\includegraphics[scale=0.40]{07D3ea_data2.eps}
\label{subfig:07D3ea_data2}
}
\subfigure[07D3ey $z=0.740$]{
\includegraphics[scale=0.40]{07D3ey_data2.eps}
\label{subfig:07D3ey_data2}
}
\subfigure[07D3gm $z=0.83$]{
\includegraphics[scale=0.40]{07D3gm_data2.eps}
\label{subfig:07D3gm_data2}
}
\end{center}
\caption{Type Ia Supernovae (CI = 4 or 5)}
\end{figure*}


\begin{figure*}
\begin{center}
\subfigure[07D3hl $z=0.67$]{
\includegraphics[scale=0.40]{07D3hl_data2.eps}
\label{subfig:07D3hl_data2}
}
\subfigure[07D3hu $z=0.572$]{
\includegraphics[scale=0.40]{07D3hu_data2.eps}
\label{subfig:07D3hu_data2}
}
\subfigure[07D3hv $z=0.351$]{
\includegraphics[scale=0.40]{07D3hv_data2.eps}
\label{subfig:07D3hv_data2}
}
\subfigure[07D3hw $z=0.748$]{
\includegraphics[scale=0.40]{07D3hw_data2.eps}
\label{subfig:07D3hw_data2}
}
\subfigure[07D3hz $z=0.506$]{
\includegraphics[scale=0.40]{07D3hz_data2.eps}
\label{subfig:07D3hz_data2}
}
\subfigure[07D3ib $z=0.681$]{
\includegraphics[scale=0.40]{07D3ib_data2.eps}
\label{subfig:07D3ib_data2}
}
\subfigure[07D3it $z=0.835$]{
\includegraphics[scale=0.40]{07D3it_data2.eps}
\label{subfig:07D3it_data2}
}
\subfigure[07D4fl $z=0.503$]{
\includegraphics[scale=0.40]{07D4fl_data2.eps}
\label{subfig:07D4fl_data2}
}
\end{center}
\caption{Type Ia Supernovae (CI = 4 or 5)}
\end{figure*}


\begin{figure*}
\begin{center}
\subfigure[08D2aa $z=0.538$]{
\includegraphics[scale=0.40]{08D2aa_data2.eps}
\label{subfig:08D2aa_data2}
}
\subfigure[08D2ad $z=0.554$]{
\includegraphics[scale=0.40]{08D2ad_data2.eps}
\label{subfig:08D2ad_data2}
}
\subfigure[08D2bj $z=0.84$]{
\includegraphics[scale=0.40]{08D2bj_data2.eps}
\label{subfig:08D2bj_data2}
}
\subfigure[08D2dr $z=0.355$]{
\includegraphics[scale=0.40]{08D2dr_data2.eps}
\label{subfig:08D2dr_data2}
}
\subfigure[08D2dz $z=0.65$]{
\includegraphics[scale=0.40]{08D2dz_data2.eps}
\label{subfig:08D2dz_data2}
}
\subfigure[08D2gw $z=0.715$]{
\includegraphics[scale=0.40]{08D2gw_data2.eps}
\label{subfig:08D2gw_data2}
}
\subfigure[08D2hw $z=0.746$]{
\includegraphics[scale=0.40]{08D2hw_data2.eps}
\label{subfig:08D2hw_data2}
}
\subfigure[08D2id $z=0.833$]{
\includegraphics[scale=0.40]{08D2id_data2.eps}
\label{subfig:08D2id_data2}
}
\end{center}
\caption{Type Ia Supernovae (CI = 4 or 5)}
\end{figure*}


\begin{figure*}
\begin{center}
\subfigure[08D2iq $z=0.709$]{
\includegraphics[scale=0.40]{08D2iq_data2.eps}
\label{subfig:08D2iq_data2}
}
\subfigure[08D2kj $z=0.702$]{
\includegraphics[scale=0.40]{08D2kj_data2.eps}
\label{subfig:08D2kj_data2}
}
\subfigure[08D3bh $z=0.52$]{
\includegraphics[scale=0.40]{08D3bh_data2.eps}
\label{subfig:08D3bh_data2}
}
\subfigure[08D3dc $z=0.799$]{
\includegraphics[scale=0.40]{08D3dc_data2.eps}
\label{subfig:08D3dc_data2}
}
\subfigure[08D3gb $z=0.17$]{
\includegraphics[scale=0.40]{08D3gb_data2.eps}
\label{subfig:08D3gb_data2}
}
\subfigure[08D3gf $z=0.352$]{
\includegraphics[scale=0.40]{08D3gf_data2.eps}
\label{subfig:08D3gf_data2}
}
\subfigure[08D3gu $z=0.767$]{
\includegraphics[scale=0.40]{08D3gu_data2.eps}
\label{subfig:08D3gu_data2}
}
\subfigure[08D3hh $z=0.452$]{
\includegraphics[scale=0.40]{08D3hh_data2.eps}
\label{subfig:08D3hh_data2}
}
\end{center}
\caption{Type Ia Supernovae (CI = 4 or 5)}
\end{figure*}
\newpage

\begin{figure*}
\begin{center}
\subfigure[06D1ck $z=0.90$]{
\includegraphics[scale=0.40]{06D1ck_data2.eps}
\label{subfig:06D1ck_data2}
}
\subfigure[06D2iz $z=0.85$]{
\includegraphics[scale=0.40]{06D2iz_data2.eps}
\label{subfig:06D2iz_data2}
}
\subfigure[06D2ji $z=0.90$]{
\includegraphics[scale=0.40]{06D2ji_data2.eps}
\label{subfig:06D2ji_data2}
}
\subfigure[06D2ju $z=0.927$]{
\includegraphics[scale=0.40]{06D2ju_data2.eps}
\label{subfig:06D2ju_data2}
}
\subfigure[06D4fc $z=0.677$]{
\includegraphics[scale=0.40]{06D4fc_data2.eps}
\label{subfig:06D4fc_data2}
}
\subfigure[07D3bo $z=0.92$]{
\includegraphics[scale=0.40]{07D3bo_data2.eps}
\label{subfig:07D3bo_data2}
}
\subfigure[07D3bt $z=0.91$]{
\includegraphics[scale=0.40]{07D3bt_data2.eps}
\label{subfig:07D3bt_data2}
}
\subfigure[07D3do $z=1.02$]{
\includegraphics[scale=0.40]{07D3do_data2.eps}
\label{subfig:07D3do_data2}
}
\end{center}
\caption{Probable Type Ia Supernovae (CI = 3)}
\end{figure*}


\begin{figure*}
\begin{center}
\subfigure[08D1aa $z=0.54$]{
\includegraphics[scale=0.40]{08D1aa_data2.eps}
\label{subfig:08D1aa_data2}
}
\subfigure[08D2ch $z=0.474$]{
\includegraphics[scale=0.40]{08D2ch_data2.eps}
\label{subfig:08D2ch_data2}
}
\subfigure[08D2cl $z=0.831$]{
\includegraphics[scale=0.40]{08D2cl_data2.eps}
\label{subfig:08D2cl_data2}
}
\subfigure[08D3dx $z=0.928$]{
\includegraphics[scale=0.40]{08D3dx_data2.eps}
\label{subfig:08D3dx_data2}
}
\end{center}
\caption{Probable Type Ia Supernovae (CI = 3)}
\end{figure*}

\newpage

\begin{figure*}
\begin{center}
\subfigure[05D4bo $z$ unknown]{
\includegraphics[scale=0.40]{05D4bo_data2.eps}
\label{subfig:05D4bo_data2}
}
\subfigure[06D1gu $z=0.87$]{
\includegraphics[scale=0.40]{06D1gu_data2.eps}
\label{subfig:06D1gu_data2}
}
\subfigure[06D1hl $z$ unknown]{
\includegraphics[scale=0.40]{06D1hl_data2.eps}
\label{subfig:06D1hl_data2}
}
\subfigure[06D1jp $z$ unknown]{
\includegraphics[scale=0.40]{06D1jp_data2.eps}
\label{subfig:06D1jp_data2}
}
\subfigure[06D3fv $z$ unknown]{
\includegraphics[scale=0.40]{06D3fv_data2.eps}
\label{subfig:06D3fv_data2}
}
\subfigure[06D3hd $z=0.2409$]{
\includegraphics[scale=0.40]{06D3hd_data2.eps}
\label{subfig:06D3hd_data2}
}
\subfigure[06D4gn $z$ unknown]{
\includegraphics[scale=0.40]{06D4gn_data2.eps}
\label{subfig:06D4gn_data2}
}
\subfigure[07D2bu $z=0.733$]{
\includegraphics[scale=0.40]{07D2bu_data2.eps}
\label{subfig:07D2bu_data2}
}
\end{center}
\caption{Unknown (CI=2)}
\end{figure*}

\begin{figure*}
\begin{center}
\subfigure[07D2ki $z=0.673$]{
\includegraphics[scale=0.40]{07D2ki_data2.eps}
\label{subfig:07D2ki_data2}
}
\subfigure[07D2kl $z=1.023$]{
\includegraphics[scale=0.40]{07D2kl_data2.eps}
\label{subfig:07D2kl_data2}
}
\subfigure[07D3bb $z$ unknown]{
\includegraphics[scale=0.40]{07D3bb_data2.eps}
\label{subfig:07D3bb_data2}
}
\subfigure[07D3bp $z=0.769$]{
\includegraphics[scale=0.40]{07D3bp_data2.eps}
\label{subfig:07D3bp_data2}
}
\subfigure[07D3fi $z$ unknown]{
\includegraphics[scale=0.40]{07D3fi_data2.eps}
\label{subfig:07D3fi_data2}
}
\subfigure[08D2au $z=0.563$]{
\includegraphics[scale=0.40]{08D2au_data2.eps}
\label{subfig:08D2au_data2}
}
\subfigure[08D3fp $z$ unknown]{
\includegraphics[scale=0.40]{08D3fp_data2.eps}
\label{subfig:08D3fp_data2}
}
\subfigure[08D3fu $z=0.426$]{
\includegraphics[scale=0.40]{08D3fu_data2.eps}
\label{subfig:08D3fu_data2}
}
\end{center}
\caption{Unknown (CI=2)}
\end{figure*}
\newpage

\begin{figure*}
\begin{center}
\subfigure[06D1dt $z=0.298$]{
\includegraphics[scale=0.40]{06D1dt_data2.eps}
\label{subfig:06D1dt_data2}
}
\subfigure[06D1gg $z$ unknown]{
\includegraphics[scale=0.40]{06D1gg_data2.eps}
\label{subfig:06D1gg_data2}
}
\subfigure[06D4hc $z=0.38$]{
\includegraphics[scale=0.40]{06D4hc_data2.eps}
\label{subfig:06D4hc_data2}
}
\subfigure[07D2ke $z=0.114$]{
\includegraphics[scale=0.40]{07D2ke_data2.eps}
\label{subfig:07D2ke_data2}
}
\subfigure[07D3ai $z=0.198$]{
\includegraphics[scale=0.40]{07D3ai_data2.eps}
\label{subfig:07D3ai_data2}
}
\subfigure[07D3am $z=0.214$]{
\includegraphics[scale=0.40]{07D3am_data2.eps}
\label{subfig:07D3am_data2}
}
\subfigure[08D2eo $z=0.125$]{
\includegraphics[scale=0.40]{08D2eo_data2.eps}
\label{subfig:08D2eo_data2}
}
\subfigure[08D2fj $z=0.507$]{
\includegraphics[scale=0.40]{08D2fj_data2.eps}
\label{subfig:08D2fj_data2}
}
\end{center}
\caption{Probably or Definitely Not Type Ia Supernovae (CI=1 or  0)}
\end{figure*}

\begin{figure*}
\begin{center}
\subfigure[08D3au $z$ unknown]{
\includegraphics[scale=0.40]{08D3au_data2.eps}
\label{subfig:08D3au_data2}
}
\end{center}
\caption{Probably or Definitely Not Type Ia Supernovae (CI=1 or  0)}
\end{figure*}

%%% Local Variables:  %%% mode: latex %%% TeX-master: "snls_spec_v3" %%% End: 
